Which Matters Most in Making Fund Investment Decisions? A Multi-granularity Graph Disentangled Learning Framework

In this paper, we highlight that both conformity and risk preference matter in making fund investment decisions beyond personal interest and seek to jointly characterize these aspects in a disentangled manner. Consequently, we develop a novel M ulti-granularity Graph Disentangled Learning framework named MGDL to effectively perform intelligent matching of fund investment products. Benefiting from the well-established fund graph and the attention module, multi-granularity user representations are derived from historical behaviors to separately express personal interest, conformity and risk preference in a fine-grained way. To attain stronger disentangled representations with specific semantics, MGDL explicitly involve two self-supervised signals, i.e., fund type based contrasts and fund popularity. Extensive experiments in offline and online environments verify the effectiveness of MGDL.

==> sec-rel.tex <==
\section{Related work}
Since the main task in our study could be generally formulated as a  classical matching or recommendation problem, we review the most related work in recommendation with behavior data and disentangled learning.

\subsection{Recommendation with Behavior Data} User behavior modelling is an effective technique widely used in recommmender systems, which takes full advantage of historical interaction records for preference and intention inference~\cite{shan2016deep,wang2021survey}. In particular, Markov Chains is the main tool in the early phase~\cite{cheng2013you}, while the emerging deep learning enhances recommender systems via  high-order feature interaction with CNN and DNN based architectures~\cite{tang2018personalized} and sequential relation extraction with RNN based components~\cite{hidasi2015session,yu2019adaptive}. Furthermore, attention mechanism~\cite{vaswani2017attention} is adopted to quantify the different importance of historical behaviors \wrt the target interaction~\cite{kang2018self,sun2019bert4rec,fan2021lighter}.

%shan2016deep,

% Inspired from the graph neural networks (GNNs), 
Inspired by the huge success of graph neural networks (GNNs),
higher-order connectivity in behavior data is naturally exploited in an end-to-end way to achieve state-of-the-art performance for recommendation~\cite{he2020lightgcn,wu2020graph}. One line of these works is devoted to architecture of the basic user-item bipartite graph mining~\cite{he2020lightgcn,wang2019neural,fan2022graph}, while another line of works mainly enrich the pure behavior data with social relations~\cite{fan2019graph} and item-side knowledge~\cite{wang2019kgat,yang2022knowledge,liu2022unify}.

In a word, these methods follow the common paradigm that learns a single representation derived from historical behaviors. Unfortunately, such a  paradigm may achieve unsatisfying performance in fund matching, where both of conformity and risk preference matter in making fund
investment decisions beyond personal interest. In our study,  we explicitly distinguish the above aspects via graph based architecture with financial scenario-specific supervised signals. 

%\paragraph{Recommendation with Graph Neural Networks.}

\subsection{Recommendation with Disentangled Learning}
Recently, disentangled learning has received considerable attentions in recommendation, especially for multi-interest extraction.
Early works achieve this goal via the neural turing machine~\cite{pi2019practice}, where the mainstream approaches realize interest decomposition with the dynamic routing and the self-attention mechanism~\cite{li2019mind,cen2020controllable}. 
With various kinds of auxiliary data in web services, several efforts are made to leveraging temporal pattern~\cite{chen2021exploring} and graph structure~\cite{ma2019disentangled,wang2020dgcf,tian2022multi} to enhance multi-interest representation. 

Although these methods achieve remarkable performance in multi-interest extraction, they are still unsuitable to our scenarios since we would involve specific semantics, \ie personal interest, conformity and risk preference. 
Besides, the lack of labeled data is the core bottleneck of current approaches. In this paper, we borrow the idea of self-supervised learning~\cite{jaiswal2020survey} to explicitly supervise risk preference and conformity with fund type based contrasts and fund popularity, respectively.

% \textbf{Sequential recommendation.} The effective learning of sequential patterns remains to be a critical issue for sequential recommendation. Traditional methods based on Markov Chains (Rendle et al. 2010; Chen et al. 2012) are exploited to predict transition from one state to another in the state
% space for sequential recommendation. Another line of work adopts recurrent neural networks (RNNs) (Hidasi et al. 2016; Beutel et al. 2018) or plain convolutional neural networks (CNNs) (Tang and Wang 2018; Yan et al. 2019; Yuan et al. 2019) to model sequential patterns.

% More recently, RNN- or CNN-based models in sequential recommendation have been gradually substituted by self- attention-based Transformer (Vaswani et al. 2017) architectures, demonstrating great success on machine translation task. Specifically, SASRec (Kang and McAuley 2018) primarily introduces such self-attention into sequential recommendation, achieving extraordinary performance. Moreover, BERT4Rec (Sun et al. 2019) employs the deep bidirectional self-attention to enhance user behavior sequence representations. SSEPT (Wu et al. 2020) poses a personalized Transformer to capture recent engagement patterns for each user. Furthermore, LightSANs (Fan et al. 2021) propose to utilize linear projections to learn latent user interests, generating self-attention-based interest-aware representations.

% \noindent\textbf{Disentangled representation learning.} Originated from the computer vision field, disentangled representation learning improves the model robostness and interpretability by separating different components in data representation\cite{Hamaguchi2019rare}. However, disentangled representation learning for recommender systems have not been well explored until recently\cite{li2019mind,cen2020controllable}.

% MIND\cite{li2019mind} introduces the capsule network\cite{Sabour2017dyna} into recommendation area and utilized the dynamic routing mechanism in capsule network to extract user's multiple interests in e-commerce scenarios. ComiRec\cite{cen2020controllable} extends the dynamic routing mechanism to self-attention mechanism\cite{Lin2017sa} for interest extraction. DICE\cite{zheng2021dice} utilizes structural causal embedding to model user's interest and conformity in interaction and it achieved remarkable performance with respect to SOTA causal recommendation methods. Further, Besides, with graph neural networks proven to be successful in many machine learning tasks, it shed light on disentangled representation learning, for example, DisenGCN\cite{ma2019disentangled} uses dynamic routing in graph neural networks to enhance the graph representation ability while DGCF\cite{wang2020dgcf} learns multiple user latent intentions by utilizing graph convolutional networks. 
